Computationally Efficient PAC RL in POMDPs with Latent Determinism and Conditional Embeddings

We study reinforcement learning with function approximation for large-scale Partially Observable Markov Decision Processes (POMDPs) where the state space and observation space are large or even continuous. Particularly, we consider Hilbert space embeddings of POMDP where the feature of latent states and the feature of observations admit a conditional Hilbert space embedding of the observation emission process, and the latent state transition is deterministic. Under the function approximation setup where the optimal latent state-action $Q$-function is linear in the state feature, and the optimal $Q$-function has a gap in actions, we provide a \emph{computationally and statistically efficient} algorithm for finding the \emph{exact optimal} policy. We show our algorithm's computational and statistical complexities scale polynomially with respect to the horizon and the intrinsic dimension of the feature on the observation space. Furthermore, we show both the deterministic latent transitions and gap assumptions are necessary to avoid statistical complexity exponential in horizon or dimension. Since our guarantee does not have an explicit dependence on the size of the state and observation spaces, our algorithm provably scales to large-scale POMDPs.

==> deterministic_pomdp.tex <==
\section{POMDP with deterministic latent transition}

Consider the finite horizon $H$ setting. We assume invertible conditional mean embedding. More formally, we have two RKHS, $\Hcal_o$ and $\Hcal_s$ which have feature mapping $\psi$ and $\phi$ accordingly.  
\begin{assum}
There exists a linear operator $K:\Hcal_s \mapsto \Hcal_o$, such that $\forall s: \EE_{o\sim O(\cdot | s)} [\psi(o)] = K \phi(s)$.
\end{assum}

We also assume that the $Q^\star$ is linear in feature $\phi$. 
\begin{assum}
For all $a\in\Acal, h\in [H]$, there exists $w^\star_{a;h}$, such that $Q_h^\star(s,a) = (w^\star_{a;h})^{\top} \phi(s), \forall s$.
\end{assum}

\wen{i think the gap condition is needed..but will see when trying out..AS: See Theorem~\ref{thm:POMDP_lower_bound} for the lower bound} 
\begin{assum}
\label{ass:gap_assumption} 
Define $\text{gap}_h(s,a) = V^\star_h(s) - Q^\star_h(s,a)$.  There exists $\alpha \in [0, H]$, such that $\min_{h, s,a} \{  \text{gap}_h(s,a): \text{gap}_h(s,a) > 0 \} \geq \alpha$.
\end{assum}

\begin{algorithm}[t] 
\caption{Deterministic POMDP} \label{alg:deterministic_pomdp}
\begin{algorithmic}[1]
  \STATE {\bf  Input:} Policy classes $\left\{ \Pi_h \subset \Acal^{h-1} \mapsto \Delta(\Acal) \right\}$ 
  \STATE Initialize datasets $\Dcal_0, \dots, \Dcal_{H-1}$
  \WHILE{true}
  	\STATE For all $h \in [H],a\in \Acal$, $\theta_{a;h} = \argmin_{\theta} \EE_{\Dcal_{a;h}} (\theta^{\top} x - y)^2 + \lambda \| \theta  \|^2_2$
	\STATE Compute $x_0 := \widehat\EE_{o\sim O(\cdot | s_0)} \psi(o) $
	\FOR{$h = 0 \to H-1$}
		\STATE Set $a_h = \argmax_{a} [ \theta_{a;h}^\top x_h]$ 
		\STATE Compute $x_{h+1} = \widehat\EE_{o\sim O(\cdot | a_{0:h})} \psi(o) $ {\textcolor{blue}{\\\#\# This can be done by repeatedly resetting to $s_0$ and executing $a_{0:h}$}}
	\ENDFOR
	\IF{ $\forall h: \|x_h\|_{\Sigma_h^{-1}} \leq \varepsilon $ }
		\STATE Return $\{a_0, \dots, a_{H-1}\}$
	\ELSE
		\STATE Find an $h$ such that $\|x_h\|_{\Sigma_h^{-1}} > \varepsilon$,   \label{alg:eliptical} 
		\FOR{  $\forall a'\in \Acal$} \label{alg:for1} 
		\STATE   Compute $x_{h+1} = \widehat\EE_{o\sim O(\cdot | a_{0:h-1}, a')} \psi(o)$,  $y_{a'} = r(a_{0:h-1},a') + \text{Compute-}V^\star(x_{h+1}, h+1; a_{0:h-1},a')$ \label{alg:start} \label{alg:bad_original}
		\STATE Add $\Dcal_{a';h} = \Dcal_{a';h} + \{ x_h,  y_{a'} \}$ \label{alg:add_data1}
		\ENDFOR \label{alg:for2} 
	\ENDIF
  \ENDWHILE
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[t] 
\caption{Compute-$V^\star$} \label{alg:compute_q_star}
\begin{algorithmic}[1]
	\IF{$h = H-1$}
		\STATE Return $\max_{a} r(a_{0:H-2},a)$ {\textcolor{blue}{\#\# it is $V^\star_{H-1}(s_{H-1})$}}
	\ELSE 
		\IF{ $\|x_{h}\|_{\Sigma^{-1}_{h}} \leq \varepsilon$} \label{alg:good}
			\STATE $\forall a$, $\hat \theta_{a;h} = \argmin_{\theta } \EE_{\Dcal_{a;h}} ( x^{\top}\theta - y)^2 + \lambda \|\theta\|_2^2$
			\STATE Compute $a_{h} = \argmax_{a} (\hat \theta_{a;h})^{\top} x_{h}$
			\STATE Compute $x_{h+1} = \widehat \EE_{o\sim O(\cdot | a_{0:h})} \psi(o)$
			\STATE Return $r(a_{0:h-1},a_h) + \text{Compute-}V^\star(x_{h+1}, h+1;  a_{0:h})$ {\textcolor{blue}{\#\# this is $\max_{a }r(s_h,a) + V_{h+1}^\star(  T(s_h,a)  )$}}
		\ELSE  \label{alg:eliptical2}
			\FOR{$ a' \in \Acal $} 
				\STATE Compute $x_{h+1} = \widehat\EE_{o\sim O(\cdot | a_{0:h-1},a')}\psi(o)$  
				\STATE $y_{a'} = r(a_{0:h-1}, a') + \text{Compute-}V^\star( x_{h+1}, h+1; \{a_{0:h-1},a'\} )$  {\textcolor{blue}{\#\# this is $Q^\star_{h}(s_{h},a')$}} \label{alg:bad}
				\STATE $\Dcal_{a';h} := \Dcal_{a';h} +  \{  x_h, y_{a'} \}$ \label{alg:add_data2}
			\ENDFOR
			\STATE Return $\max_{a} y_{a'}$   {\textcolor{blue}{\#\# this is $V^\star_{h}(s_{h})$}}
		\ENDIF
	\ENDIF 
	
\end{algorithmic}
\end{algorithm}

In the algorithm, executing a sequence of actions $a_{0:h}$ will lead to $s_{h+1}$. Since $s_{h+1}$ is not observable, we use its observable quantity $ \overline x_{h+1} := \EE_{o\sim O(\cdot | a_{0:h})} \psi(o)$ to represent it. However, we can only approximate this expectation via finite samples. We denote $x_{h+1} = \widehat{\EE}_{o\sim O(\cdot | a_{0:h})} \psi(o)$ as the empirical estimate of $\overline x_{h+1}$. Note that since the system is deterministic, we can repeatedly execute $a_{0:h}$ to reach $s_{h+1}$ and generate $o\sim O(\cdot | s_{h+1})$.  Let us denote the difference between $\overline x_{h}$ and $x_h$ as $\| \overline x_h - x_h \|_2 \leq \xi$ (note that $\xi$ shrinks in the rate of $1/\sqrt{n}$ with $n$ being the number of samples for $\widehat \EE$). 

We first use the following lemma to analyze the linear regression. 
\begin{lemma}[Linear Regression]
Consider a sequence of covariates $x_1,\dots, x_n$ such that $\EE[ x_i | x_{1:i-1}] = \overline x_i$, and $ \max_{w:\|w\|_2\leq 1} w^{\top} ( \overline x_i - x_i ) \leq \zeta$. Assume $y_i = (\theta^\star)^{\top} \overline x_i $, for all $i$.  Denote $\theta := \Sigma^{-1} \sum_{i=1}^n x_i y_i$, where $\Sigma = \sum_{i=1}^n x_i x_i^{\top} + \lambda I$. With probability at least $1-\delta$, we have:
\begin{align*}
\left\| \theta - \theta^\star \right\|_{\Sigma} \leq \sqrt{\lambda} \|\theta^\star\|_2 + \|\theta^\star\|_2 \zeta \sqrt{ d\ln\left(    1 + n /\lambda  \right)  + \ln (1/\delta)}. 
\end{align*}
\end{lemma} 
\begin{proof}
\begin{align*}
\theta  & = \Sigma^{-1} \sum_{i=1}^n x_i ( \overline x_i^{\top} \theta^\star)  = \Sigma^{-1} \sum_{i=1}^n x_i \left( (x_i)^{\top} \theta^\star + ( \overline x_i - x_i)^{\top} \theta^\star  \right) \\
& = \theta^\star - \lambda \Sigma^{-1} \theta^\star + \Sigma^{-1}\sum x_i (\overline x_i - x_i)^{\top} \theta^\star
\end{align*}
Hence, for $\|\theta - \theta^\star\|^2_{\Sigma}$, we have:
\begin{align*} 
\sqrt{ (\theta - \theta^\star)^{\top}  \Sigma (\theta - \theta^\star) } \leq  \sqrt{\lambda} \|\theta^\star\|_2 + \|\theta^\star\|_2 \zeta \sqrt{ d\ln\left(    1 + n /\lambda  \right)  + \ln (1/\delta)} 
\end{align*}

--------------

\begin{align*}
   \| \sum x_i(\bar x_i-x_i)^{\top}\theta^\star \|_{\Sigma^{-1}} \leq    \| \sum x_i \epsilon^{\top}_i \theta^\star  \|_{\Sigma^{-1}} \leq  \zeta \|\theta^\star\|_2 \sqrt{ d\ln\left(    1 + n /\lambda  \right)  + \ln (1/\delta)} 
\end{align*}
Here, we use $\epsilon^{\top}_i \theta^{*}$ is $\zeta\|\theta^{\star}\|$-sub Gaussian. 



\end{proof}


The following lemma shows that $\text{Compute-}Q^\star(x, a, h; a_{0:h-1})$ always return $Q_h^\star(s_{h}, a)$ where $s_h$ is the state reached by the sequence of actions $a_{0:h-1}$.
\ascomment{We should use \(\Delta\) to denote the gap} 
\begin{lemma}[The accuracy of $\text{Compute-}V^\star$] When $\varepsilon = \sigma / (2 \| \theta^\star \|_2 (1 + \sqrt{d}))$ and $\xi \leq \sigma / 2$, we have that for any $x$, $\text{Compute-}V^\star(x, h; a_{0:h-1}) = V^\star_h(s_h)$ where $s_h$ is the state reached by $a_{0:h-1}$. 
\end{lemma}
\begin{proof}
We prove by induction. When $h = H-1$, our procedure simply returns $\max_a r(s_{H-1}, a)$ by querying the reward function directly, which is equal to $V^\star_{H-1}(s_{H-1})$ by definition. 

Now assume that conclusion holds at $h+1$. We prove the same for $h$. 

There are two cases, the first case is $\|x_{h}\|_{\Sigma^{-1}_{h}} > \varepsilon$. In this case, we calculate $Q^\star_h(s_h, a')$ for all $a' \in \Acal$ via calling $\text{Compute-}V^\star$ at layer $h+1$ with actions $\{a_{0:h-1}, a'\}$. Note that by inductive hypothesis, we have $\text{Compute-}V^\star(x_{h+1}, h+1; a_{0:h-1},a') = V^\star(s_{h+1})$ with $s_{h+1}$ being the state reached by $a_{0:h-1},a'$. Thus, it is easy to verify that $y_{a'} = Q^\star_h(s_h, a')$, and thus $\max_{a'} y_{a'} = V^\star_h(s_h)$.  

The second case is $\|x_{h}\|_{\Sigma^{-1}_{h}} \leq \varepsilon$.  Recall that $Q^\star_h(s,a) =( \theta_{a;h}^\star)^{\top} \overline x_{h}$ via linear regression result, we know that:
\begin{align*}
\forall a: \left\lvert \hat \theta_{a:h}^{\top} x_{h} - (\theta_{a;h}^\star)^{\top} \overline{x}_{h}   \right\rvert  & \leq \left\lvert (\hat \theta_{a;h} - \theta^\star_{a;h})^{\top} x_{h}  \right\rvert + \left\lvert  (\theta^\star_{a;h})^{\top} ( x_{h} - \overline x_{h})        \right\rvert \\
& \lesssim ( \|\theta^\star \|_2 ( 1 +  \sqrt{ d } ) ) \varepsilon + \|\theta^\star\|_2 \zeta. 
\end{align*}
Thus, when $\varepsilon \lesssim  \frac{\sigma}{2 \|\theta^\star\|_2 (1 + \sqrt{d}) }$, and $\xi \lesssim \sigma / 2$, we have that:
\begin{align*}
\forall a: \left\lvert \hat \theta_{a:h}^{\top} x_{h} - (\theta_{a;h}^\star)^{\top} \overline{x}_{h}   \right\rvert \leq \sigma / 2.
\end{align*}
Together with the gap assumption, this means that $\argmax_{a} \hat \theta_{a:h}^{\top } x_{h} = \argmax_{a} (\theta^\star_{a;h})^{\top} \overline x_{h}$. To complete the proof, note that we use $a_{h} := \argmax_{a} \hat \theta_{a:h}^{\top } x_{h}$ as the action at $h$, and then query $\text{Compute-}V^\star(x_{h+1}, h+1; \{a_{h-1}, a_h\})$, which by inductive hypothesis should return $V^\star_{h+1}(s_{h+1})$ with $s_{h+1}$ being the state reached by $\{a_{h-1},a_h\}$. 
\end{proof}

The next lemma shows that when the algorithm terminates, we must find a near optimal policy. 
\begin{lemma}[Near optimality upon termination] Algorithm~\ref{alg:deterministic_pomdp} returns an optimal policy on termination.
\end{lemma}
\begin{proof}
Denote $\tau = \{s_h^\star, a_h^\star\}_{h=0}^{H-1}$ as the optimal trajectory. 
Upon termination of Algorithm~\ref{alg:deterministic_pomdp}, we have $\forall h: \|x_h\|_{\Sigma_h^{-1}} \leq \varepsilon$. We prove the theorem by induction. At $h=0$, we know that $s_0 = s_0^\star$. By our linear regression guarantee, and the value of $\varepsilon$, we know that for all $a\in \Acal$, 
\begin{align*}
\left\lvert  \theta_{a;0}^{\top} x_0 - (\theta^\star_{a;0})^{\top} \overline x_0   \right\rvert \leq \sigma / 2,
\end{align*} which means that $a_0 = \argmax_{a} \theta_{a;0}^{\top} x_h = a_0^\star$ (i.e., $a_\tau = a_\tau^\star$ for $\tau \leq h$). This completes the base case. 
Now assume it holds for $\tau = 0, \dots, h$. We prove for step $h+1$. Since $s_h = s_h^\star$, we have $x_h$ being an unbiased estimate of $\overline x_h$ which is $\EE_{o\sim O(\cdot | s_h^\star)} \psi(o)$. Thus, we can again use the linear regression guarantee to show that the prediction error for all $a$ must be less than $\sigma / 2$, which indicates that at $h+1$, we will pick the correct action $a_{h+1}^\star$. This completes the proof. 
\end{proof}


\begin{theorem}
Algorithm~\ref{alg:deterministic_pomdp} terminates in $O(M|\Acal|H^3d/\epsilon^2)$ time.  
\end{theorem}

\begin{proof}
~
\paragraph{The number of times we call Line \ref{alg:eliptical} in Algorithm \ref{alg:deterministic_pomdp}   at layer $h$ is upper-bounded by $d/\epsilon^2$}

At horizon $h$, when the new data $x_h$ is added, we always have $\|x_h\|_{\Sigma_h}^{-1}>\epsilon$ (Line \ref{alg:eliptical} in Algorithm \ref{alg:deterministic_pomdp} or Line \ref{alg:eliptical2} in Algorithm \ref{alg:compute_q_star}). Letting the total number we call Line \ref{alg:eliptical} in Algorithm \ref{alg:deterministic_pomdp} and Line \ref{alg:eliptical2} in Algorithm \ref{alg:compute_q_star} be $N$, we have
\begin{align*}
   \sum_{i=1}^{N} \|x^{(i)}_h\|_{\Sigma_h}^{-1}\leq \sqrt{Nd}
\end{align*}
where $i$ is the index for data. Thus, the following holds  
\begin{align*}
    \epsilon N \leq \sqrt{Nd}
\end{align*}
This implies $N$ is upper-bounded by $d/\epsilon^2$. Thus, the number of we call  Line \ref{alg:eliptical} in Algorithm \ref{alg:deterministic_pomdp} is upper-bounded by  $d/\epsilon^2$. 

~
\paragraph{Argument for total running time}

When we call Line \ref{alg:eliptical} in Algorithm \ref{alg:deterministic_pomdp}, we consider the running from Line \ref{alg:for1} to  \ref{alg:for2}. Let $m-1$ be the number of times we already visit Line \ref{alg:eliptical} in Algorithm \ref{alg:deterministic_pomdp}. 

Hereafter, we consider the case at iteration $m$. When we visit Line \ref{alg:start} in Algorithm \ref{alg:deterministic_pomdp}, we need to start the recursion step in Algorithm \ref{alg:compute_q_star}. This recursion is repeated in a DFS manner from $h$ to $H-1$ as in \pref{fig:illustration}. When the algorithm moves from some layer to another layer, the algorithm calls Line \ref{alg:good} or Line \ref{alg:eliptical2}, i.e., Line \ref{alg:bad} $|A|$ times in Algorithm \ref{alg:compute_q_star}. Let the number of total times the algorithm calls Line \ref{alg:good} in Algorithm \ref{alg:compute_q_star} ($g$ in \pref{fig:illustration}) be $\alpha_m$. Let the number of times the algorithm visits  Line \ref{alg:bad} in Algorithm \ref{alg:compute_q_star} and Line \ref{alg:bad_original} in Algorithm \ref{alg:deterministic_pomdp}  ($b_a$ in \pref{fig:illustration})  be  $\beta_{m}$, respectively. Then, the total running time is upper-bounded by 
\begin{align*}
  \sum_{m=1}^{Hd/\epsilon^2} M H\{ \alpha_{m}+\beta_{m} \}. 
\end{align*}
Note $H$ is the number of times we need to reset and $M$ is the number of samples in $\hat E$. 

Next, we show $\alpha_{m}\leq H\beta_{m}+H $. First, we denote a set of all $g$ and $b_a$ nodes the algorithm traverse at iteration $m$ in the tree by $G_m$ and $B_m$, respectively. We denote a subgraph on the tree consisting of nodes and edges which the algorithm traverses by $\tilde \Omega_m$. We denote a subgraph in $\tilde \Omega_m$ consisting of nodes $G_m$ and edges whose both sides belong to $G_m$ by $\tilde G_m$.  We divide $\tilde G_m$ into connected components on $\tilde \Omega_m$. Here, each component has at most $H$ nodes. The most upstream node in a component is adjacent to some node in $B_m$ on $\tilde \Omega_m$. Besides, this node in $B_m$ is not shared by other connected components in $\tilde G_m$. This ensures that  $\alpha_{m}\leq H\beta_{m} $.

Finally, we use $\sum_{m=1}^{Hd/\epsilon^2}  \beta_{m}\leq |\Acal|Hd/\epsilon^2$ as we see the number of times we call Line \ref{alg:eliptical} in Algorithm \ref{alg:deterministic_pomdp} and Line \ref{alg:eliptical2} in Algorithm \ref{alg:compute_q_star} is upper-bounded by $Hd/\epsilon^2$. 
Thus, 
\begin{align*}
      \sum_{m=1}^{Hd/\epsilon^2} MH\{ \alpha_{m}+\beta_{m} \}\leq    M\sum_{m=1}^{Hd/\epsilon^2} H\{  H \beta_{m}+H \} \leq MH(H+1)H|\Acal| d/\epsilon^2. 
\end{align*}

\end{proof}


\begin{figure}[!t]
    \centering
    \includegraphics[width = 0.7\textwidth]{pomdp.png}
    \label{fig:illustration}
    \caption{The root node corresponds to Line \ref{alg:start} in Algorithm \ref{alg:deterministic_pomdp}. We denote Line \ref{alg:good} in Algorithm \ref{alg:compute_q_star} by $g$. We denote line \ref{alg:bad} in Algorithm \ref{alg:compute_q_star} and Line \ref{alg:bad_original} in Algorithm \ref{alg:compute_q_star} corresponding to $a \in \Acal$ by $b_a$. In the illustration, we set $|\Acal|=3$. The example of paths the algorithm traverse is marked in orange. This corresponds to a graph $\tilde \Omega_m$. $\alpha_m$ is the total number of times the algorithm visits $g$ at iteration $m$. $\beta_m$ is the total number of times the algorithm visits $\{b_a\}$ at iteration $m$.   }
    \label{fig:my_label}
\end{figure}

-------------- 

\subsection{Lower bounds}
In this section, we will show via a lower bound that \pref{ass:gap_assumption} is necessary to get a polynomial sample complexity. Our lower bound construction is based on the lower bounds in \cite{weisz2021tensorplan}, and consists of an underlying deterministic dynamics (on the state space) with stochastic rewards. We recall the following result from their paper: 


\begin{theorem}[Lower bound for planners / MDP setting] 
\label{thm:gellerts_lower_bound}
Suppose the learner is given global access to the features \(\varphi: \Scal \times \Acal \mapsto \mathbb{R}^{d}\). Furthermore, let \(\delta, B, d, H\) be large enough constants. There exists a class \(\Mcal\) of deterministic MDPs (with stochastic rewards) with action space \(\Acal\) such that \(\abs*{\Acal} = d^{1/4} \wedge H^{1/2}\) and linearly realizable \(Q^*\) w.r.t. features \(\varphi\), such that any online planner that even has the ability to query a simulator at any state and action of its choice, must query at least
\begin{align*} 
2^{\Omega(d^{1/4} \wedge H^{1/2})}
\end{align*} samples to find a \(\delta\)-optimal policy for some MDP in this class. Since, learning is harder than planning, the lower bound extends to the online learning setting as well. 
\end{theorem}

The above lower bound can be immediately extended to our POMDP setting. However, we need to take care of the fact that in our setting the features only depend on the states whereas in the above lower bound, the features depend on both state and actions. This can be easily fixed for finite actions setting thus resulting in the following lower bound. 

\begin{theorem} 
\label{thm:POMDP_lower_bound} 
Let \(\delta, B, d, H\) be sufficiently large constants. Fix an action space \(\Acal\), state space \(\Scal\) and observation space \(\Ocal\). Furthermore, let \(\phi: \Scal \mapsto R^d\) and \(\psi: \Ocal \mapsto R^d\) be some state and observation feature vectors respectively. There exists a class of POMDPs \(\Pcal\) such that any POMDP P = $\langle \Scal, \Ocal, \Acal, T, O, r, s_0, \phi, \psi \rangle$ in this class satisfies: 
\begin{enumerate}[label=$(\alph*)$]
    \item (POMDP assumption) For any state \(s\), \(    \En_{o \sim O(\cdot \mid S)} \brk*{\psi(o)} = \phi(s),\) and 
    \item (Linear Q*) For any \(a\), there exists a \(w_a\) such that for any \(s\), \(Q^*(s, a) = (w^*_{a})^\top \phi(s). \)
\end{enumerate}
Furthermore, any learning algorithm that returns an \(\epsilon\)-optimal policy for the above family of POMDPs must collect at least 
\begin{align*}
\frac{1}{d^{1/5} \wedge H^{1/2}} 2^{\Omega \prn*{d^{1/5} \wedge H^{1/2}}}. 
\end{align*}

samples for some POMDP in \(\Pcal\). 
\end{theorem}
\begin{proof} The proof follows by lifting the class of MDPS \(\Mcal\) in Theorem~\ref{thm:gellerts_lower_bound} to POMDPs. Consider any MDP \(M = (\Scal, \Acal, T, H, d', s_0, \varphi) \in \Mcal\). Note that the construction of \(\Mcal\) guarantees that for \(M \in \Mcal\), 
\begin{enumerate}[label=\((\alph*)\)]
    \item For any \(a\), there exists a \(w\) such that for any \(s\), \(Q^*(s, a) = w^\top \varphi(s, a). \) \item There exists a stochastic reward function \(r(s, a)\) for any \(\sa\). 
    \item $|\Acal| = d'^{1/4} \wedge H^{1/2}$. 
\end{enumerate}

In the following, we define a POMDP $P_M$ based on $M$. The underlying dynamics on the state space remains the same. We first define the feature vector corresponding to states \(\Scal\). Since the number of actions are finite, we have 
\begin{align*}
\phi(s) = \prn{\prn{\varphi(s, a), \En \brk*{r(s, a)}}_{a \in \Acal}}. 
\end{align*}
Clearly, the dimensionality of the above feature is \(d = (d' + 1) \abs{A} = (d' + 1) (d'^{1/4} \wedge H^{1/2}) \leq 2 d'^{5/4} \wedge d'H^{1/2})\). Furthermore, defining \(w_a = \prn{(w \ind\crl{a' = a}, 0)_{a' \in \Acal}} \), we note that
\begin{align}
Q^*(s, a) = w^\top \varphi(s, a) &= \tri*{\prn{(w \ind\crl{a' = a}, 0)_{a' \in \Acal}}, \prn{\prn{\varphi(s, a), \En \brk*{r(s, a)}}_{a \in \Acal}}} \notag \\ 
&= w_a^\top \phi(s), \label{eq:lower_bound_POMDP1} 
\end{align}  and thus we also satisfy linear \(Q^*\) property according to the new features \(\phi\).  ~\\ 

The emission distribution partitions the observation space such that each \(O\) is associated with one state \(s\) only. The features corresponding to observations associated with states \(s\) are defined as 
\begin{align*}
    \psi(o) =  \prn{\prn{\varphi(s, a), r(s, a)}_{a \in \Acal}}.
\end{align*}
Since the rewards are stochastic, the observations above are also stochastic and clearly we have that 
\begin{align}
\En_{o \sim O(\cdot \mid s)} \brk*{\psi(o)} = \phi(s). \label{eq:lower_bound_POMDP2}
\end{align}

Thus, from \pref{eq:lower_bound_POMDP1} and  \pref{eq:lower_bound_POMDP2} the POMDP \(P_M\) constructed above satisfies the desired properties. Similarly, we can lift every MDP \(M \in \Mcal\) to construct the POMDP class \(\Pcal\). Clearly, we are not revealing any new information in the above POMDP construction which could not be accessed by making \(\Acal\) many calls to the underlying deterministic MDP (all actions same so far but a different action at the last step). Thus, from the query complexity lower bound in Theorem~\ref{thm:gellerts_lower_bound}, we immediately get that there must exist some POMDP in the class \(\Pcal\) for which we need to collect at least
\begin{align*}
\frac{1}{\abs{\Acal}} 2^{\Omega(d'^{1/4} \wedge H^{1/2})}
\end{align*}
many samples. Plugging in the relation \(d = d'^{5/4} \wedge H^{1/2}\) in the above, we get the lower bound
\begin{align*}
\frac{1}{d^{1/5} \wedge H^{1/2}} 2^{\Omega \prn*{d^{1/5} \wedge H^{1/2}}}. 
\end{align*}

\end{proof}

\section{Hilbert Space Embeddings}



\subsection{Algorithm} 

Let $k_{\Ocal}(\cdot,\cdot)$ be a kernel over the observation space. 

We define 
\begin{align*}
    & \mu_h(a_{0:h-1},Z(a_{0:h-1}),\Dcal_{a,h})   =   \hat \kb(a_{0:h-1},Z(a_{0:h-1}),\Dcal_{a,h})^{\top}(\hat \Kb(\Dcal_{a,h}) +\lambda I)^{-1}\Yb(\Dcal_{a,h}), \\ 
   & \hat \sigma^2_h(\{a_{0:h-1}\},\Dcal_{a,h}) = \hat k(\{a_{0:h-1},Z(a_{0:h-1})\},\{a_{0:h-1},Z(a_{0:h-1})\})\\&-\|\hat \kb(a_{0:h-1},Z(a_{0:h-1}),\Dcal_{a,h})\|^2_{(\hat \Kb(\Dcal_{a,h}) +\lambda I)^{-1}}. 
\end{align*}

The data $\Dcal_{a,h}$ consists of $\{x,Z(x),y\}$. Then, we define
\begin{align*}
   & \hat k \prns{\{x,Z(x)\}, \{x',Z(x')\}} =  1/| Z(x)Z(x')| \sum_{z_i \in Z(x), z'_j \in Z(x')} k_{\Ocal}( z_i ,z'_j), \\ 
   & \hat \kb(x,Z(x), \Dcal_{a,h})=\{ \hat k(\{x,Z(x)\}, \{x_i,Z(x_i)\}) \}_{i=1}^{|\Dcal_{a,h}|},\\
   & \hat \Kb(\Dcal_{a:h}) =\{\hat k \prns{\{x_i,Z(x_i)\}, \{x'_j,Z(x'_j)\}} \}_{i,j}^{|\Dcal_{a,h}|,|\Dcal_{a,h}| }, \\
   & \Yb(\Dcal_{a,h}) = \{ y_i\}_{i=1}^{|\Dcal_{a,h}|}. 
\end{align*}


\begin{algorithm}[t] 
\caption{Deterministic POMDP} \label{alg:deterministic_pomdp}
\begin{algorithmic}[1]
  \STATE Initialize datasets $\Dcal_0, \dots, \Dcal_{H-1}$
  \WHILE{true}
	\FOR{$h = 0 \to H-1$}
	    \STATE Collect $Z(\{ a_{0:h-1}\}) \sim O(\cdot \mid \{ a_{0:h-1}\})$
		\STATE Set $a_h = \argmax_{a} \mu_h(a_{0:h-1},Z( a_{0:h-1}),\Dcal_{a,h})$ 
	\ENDFOR
	\IF{ $\forall h: \sigma_h(a_{0:h-1},Z( a_{0:h-1}),\Dcal_{a,h})  \leq \varepsilon $ }
		\STATE Return $\{a_0, \dots, a_{H-1}\}$
	\ELSE
		\STATE Find an $h$ such that $ \sigma_h(a_{0:h-1},Z( a_{0:h-1}),\Dcal_{a,h})  > \varepsilon$,   \label{alg:eliptical} 
		\FOR{  $\forall a'\in \Acal$} \label{alg:for1} 
		\STATE   Compute $y_{a'} = r(a_{0:h-1},a') + \text{Compute-}V^\star(h+1; \{a_{0:h-1},a'\})$ \label{alg:start} \label{alg:bad_original}
		\STATE Add $\Dcal_{a';h} = \Dcal_{a';h} + \{  a_{0:h-1}, Z( a_{0:h-1}), y_{a'} \}$ \label{alg:add_data1}
		\ENDFOR \label{alg:for2} 
	\ENDIF
  \ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t] 
\caption{Compute-$V^\star$} \label{alg:compute_q_star}
\begin{algorithmic}[1]
  \STATE {\bf  Input:} horizon $h$, state $a_{0:h-1}$
	\IF{$h = H-1$}
		\STATE Return $\max_{a} r(a_{0:H-2},a)$ {\textcolor{blue}{\#\# it is $V^\star_{H-1}(s_{H-1})$}}
	\ELSE 
	    \STATE Collect $Z(\{ a_{0:h-1}\}) \sim O(\cdot \mid \{ a_{0:h-1}\})$
		\IF{ $\sigma_h(a_{0:h-1},Z( a_{0:h-1}),\Dcal_{a,h})  \leq \varepsilon$} \label{alg:good}
		    \STATE Set $a_h = \argmax_{a} \mu_h(a_{0:h-1},Z( a_{0:h-1}),\Dcal_{a,h})$ 
			\STATE Return $r(a_{0:h-1},a_h) + \text{Compute-}V^\star(h+1; \{a_{0:h-1},a_h\})$ {\textcolor{blue}{\#\# this is $\max_{a }r(s_h,a) + V_{h+1}^\star(  T(s_h,a)  )$}}
		\ELSE  \label{alg:eliptical2}
			\FOR{$ a' \in \Acal $} 
				\STATE $y_{a'} = r(a_{0:h-1}, a') + \text{Compute-}V^\star( h+1; \{a_{0:h-1},a'\} )$  {\textcolor{blue}{\#\# this is $Q^\star_{h}(s_{h},a')$}} \label{alg:bad}
				\STATE $\Dcal_{a';h} := \Dcal_{a';h} +  \{ a_{0:h-1},Z( a_{0:h-1}), y_{a'} \}$ \label{alg:add_data2}
			\ENDFOR
			\STATE Return $\max_{a} y_{a}$   {\textcolor{blue}{\#\# this is $V^\star_{h}(s_{h})$}}
		\ENDIF
	\ENDIF
	
\end{algorithmic}
\end{algorithm}


\subsection{Theory}


Let $k_{\Scal}(\cdot,\cdot)$ be a (positive-definite) kernel over a state space. We denote the corresponding RKHS as $\Hcal_{\Scal}$. We denote the corresponding feature vector by $\phi(\cdot)$. Here for any $f \in \Fcal$, there exists $\{a_i\}$ such that $f=\sum_i a_i \phi_{i}$ and the following holds
\begin{align*}
   \EE_{s \sim u(s)}[\phi_i(s)\phi_i(s)]=\mu_i, \quad \EE_{s \sim u(s)}[\phi_i(s)\phi_j(s)]=0 (i\neq j). 
\end{align*}
Let $\bar \phi = \{\phi_i/\sqrt{\mu_i}\}$. Besides, we have $k(\cdot,\cdot) =\sum_i \phi_i(\cdot)\phi_i(\cdot)$ and  $    \langle f, g\rangle_{\Hcal_{\Scal}} = \langle \sum_i a_i \phi_{i}, \sum_i b_i \phi_{i}\rangle_{\Hcal_{\Scal}} = \sum_i a_i b_i. $



Let $k_{\Ocal}(\cdot,\cdot)$ be a(positive-definite) kernel over the oversational space with feature $\psi(o)$. We can consider the following kernel $E_{o \sim z(s),o'\sim z(s')}[k_{\Ocal}(o,o')]$ over $\Scal$. We denote this kernel by $\bar k(\cdot,\cdot)$ and the corresponding RKHS by $\Hcal_{\bar \Scal}$. 

The following assumption is equivalent to the existence of linear mean embedding operator. 
\begin{assum}
$\bar k(\cdot,s) \in \Hcal_{\Scal}$ for any $s \in \Scal$. 
\end{assum}
This just implies $\Hcal_{\bar \Scal} \subset \Hcal_{\Scal}$. Instead, we need the following stronger assumption. 
\begin{assum}
 $\Hcal_{\bar \Scal} = \Hcal_{\Scal}$ and  
\begin{align*}
   \sup_{\|p\|_2 = 1} \frac{p^{\top}\EE_{s \sim u(o)}[\bar \psi(o)\bar \psi(o)^{\top}]p}{p^{\top}\EE_{u \sim u(s)}[\EE[\bar \psi(o)\mid s]\EE[\bar \psi(o)\mid s]^{\top}]p}<c. 
\end{align*}
\end{assum} 

\begin{lemma}
Given $a^{\top}\phi(s)$ s.t. $\|a\|\leq 1$, there exists $b$ s.t. $a^{\top}\phi(s)=b^{\top}\EE[\psi(o)\mid s]$ and $\|b\|\leq c$.  
\end{lemma}
\begin{proof}
From the assumption, for any element in $\Hcal_{\bar \Scal}$ has the following representation:$
    \sum_i \alpha_i \bar k(\cdot,s_i). $ This is equal to 
\begin{align*} \textstyle
    \sum_i \alpha_i \bar k(\cdot,s_i) = \sum_i \alpha_i \EE_{o \sim Z(\cdot)}[\psi(o) ]^{\top}\EE_{o \sim Z(s_i)}[\psi(o) ]. 
\end{align*}
Thus, for any $a^{\top}\phi(s)\in \Kcal_{\Scal}$, there exists $b$ s.t. $a^{\top}\phi(s)=b^{\top}\EE[\psi(o)\mid s] $. 

Next, we prove $\|b\|\leq c$. This is proved by 
\begin{align*}
   1 = \EE_{s \sim u(s)}[\{a^{\top} \bar \phi(s)\}^2] = \EE_{s \sim u(s)}[ \{b^{\top}\EE[\psi(o)\mid s]\}^2 ] \geq 1/c  \{b^{\top}\EE_{s \sim u(o)}[\psi(o)]\}^2 =1/c \|b\|^2. 
\end{align*}


\end{proof}

Recall our assumption is $Q^{\star}_h(\cdot,a) \in \Hcal_{\Scal}$. From the assumption, $Q^{\star}_h(\cdot,a) \in \Hcal_{\bar \Scal}$. The challenge here is we cannot use $\bar k(\cdot,\cdot)$. We can only obtain $\hat k(s,s)$:
\begin{align*}
    \hat k(s,s') = \hat \EE_{o \sim O(s),o'\sim O(s')}[k_{\Ocal}(o,o')],\, \hat k_1(s,s') =  \EE_{o \sim O(s)}\hat \EE_{o'\sim O(s')}[k_{\Ocal}(o,o')], \hat k_2(s,s') \\=  \EE_{o' \sim O(s')}\hat \EE_{o \sim O(s)}[k_{\Ocal}(o,o')]. 
\end{align*}
In high probability, we have
\begin{align*}
    \{\hat k(s^{(i)},s^{(i)}) -\hat k_1(s^{(i)},s^{(i)}) -\hat k_2(s^{(i)},s^{(i)}) + \bar k(s^{(i)},s^{(i)}) \}\leq \zeta^2. 
\end{align*}
We define a feature vector $\xi(s) = \EE_{o \sim s}[\psi(o)], \hat \xi(s) = \hat \EE_{o \sim s}[\psi(o)]$. Then, $ \hat k(s,s') =\hat \xi(s)^{\top} \hat \xi(s)$ and $ \bar k(s,s') =\ \xi(s)^{\top}\xi(s)$. 

We use a dual representation. Let $Q^{\star}_h(\cdot,a)=\theta^{\star}\phi(s)$. Then, 
\begin{align*}
    \mu_h(s)= \hat \xi^{\top}(s)\hat \theta,\quad \hat \theta =(\Sigma + \lambda I)^{-1}\sum_i y^{(i)}\hat \xi(s^{(i)})
\end{align*}
where $\Sigma = \sum_i  \hat \xi(s^{(i)})\hat \xi(s^{(i)})^{\top}+\lambda I$. 


We have the following lemma.
\begin{lemma}
$ | (\hat \xi(s^{(i)}) - \xi(s^{(i)}))^{\top}\theta^{\star}| \leq  \zeta \|\theta^{\star}\|_2$ . 
\end{lemma}
\begin{proof}
\begin{align*}
   | (\hat \xi(s^{(i)}) - \xi(s^{(i)}))^{\top}\theta^{\star}| & \leq \| \hat \xi(s^{(i)}) - \xi(s^{(i)} )\|_2 \|\theta^{\star}\|_2 \\
   &\leq \{\hat k(s^{(i)},s^{(i)}) - \hat k_1(s^{(i)},s^{(i)})-\hat k_2(s^{(i)},s^{(i)}) + \bar k(s^{(i)},s^{(i)}) \}^{1/2}  \|\theta^{\star}\|_2. 
\end{align*}

\end{proof}

\begin{lemma}[Regression guarantee]
\begin{align*}
    \|\hat \theta - \theta^{\star}\|_{\Sigma}\leq \sqrt{\lambda}\|\theta^{\star}\|_2+\|\theta^{\star}\|_2 \zeta \sqrt{\gamma_{|\Dcal_{a:h}|} +1+\log(1/\delta) }
\end{align*}
\end{lemma}
\begin{proof}
We consider 
\begin{align*}
    \|\sum \xi(s_i)\{\theta^{\star}\}^{\top} (  \hat \xi(s_i)-\xi(s_i))\|_{\Sigma^{-1}}
\end{align*}
Here,
\begin{align*}
    \{\theta^{\star}\}^{\top} (  \hat \xi(s_i)-\xi(s_i))
\end{align*}
is $\zeta \|\theta^{\star}\|_2 $-sub Gaussian. 
\end{proof}


\begin{lemma}[Regression guarantee2]
When $\lambda^{-1/2}\sigma(s;\Dcal_{a:h})<\epsilon$, we have 
\begin{align*}
    |\hat \theta^{\top}\hat \xi(s)-\theta^{\star}\xi(s)|\leq \epsilon \|\hat \theta-\theta^{\star}\|_{\Sigma} +  \zeta \|\theta^{\star}\|_2. 
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
     |\hat \theta^{\top}\hat \xi(s)-\theta^{\star}\xi(s)|\leq   |\hat \theta^{\top}\hat \xi(s)-\theta^{\star}\hat \xi(s)|+  |\theta^{\star}\hat \xi(s)-\theta^{\star}\xi^{\star}(s)|. 
\end{align*}
Here,
\begin{align*}
     |\hat \theta^{\top}\hat \xi(s)-\theta^{\star}\hat \xi(s)|\leq \|\hat \theta-\theta^{\star}\|_{\Sigma}\|\hat \xi(s)\|_{\Sigma^{-1}}. 
\end{align*}
By some algebra, we have $ \|\hat \xi(s)\|_{\Sigma^{-1}} \leq \sigma(s;\Dcal_{a:h})$. 
\end{proof}

\subsection{Continuous Action}

Consider a model:$Q^{\star}(s,a) = \eta(a)^{\top}M^{*}\phi(s). $ Note this is also written as $Q^{\star}(s,a) =\theta^{\top}(\eta(a)\otimes \phi(s))$.  

    
In this case, we can still ensure $Q^{\star}(s,a) = \eta(a)M^{*}K^{\dagger}_1\EE_{o\sim s}[\psi(o)]$ when $K_1$ is left-invertible. 
Everything works by changing “for $a'\in \Acal$" to “for $a'\in \bar \Acal$", where $\bar \Acal$ is a support of $\nu$: 
\begin{align*}
    \argmax_{\nu \in \Delta(\Acal)}\log \det(\EE_{a \sim \nu}\eta(a)\eta(a)^{\top}).  
\end{align*}
Note $|\bar \Acal|\leq d(d+1)/2$ (D-optimal design). In bad events, after getting data $\{\eta(a'),y_{a'}\}$ for $a'\in \bar \Acal$, since $y_a$ is linear in $\eta(a)$ with no noise, by running regression, we can exactly estimate $\{\eta(a),y_a\}$ for any $a\in \Acal$. 

Here is a summary of change:
\begin{itemize}
    \item We need to store $\{\phi(a_{0:h-1}),\eta(a'),y_{a'}\}$ for $a'\in \bar \Acal$.
    \item The elliptical potential is defined using a feature $ \phi(s) \otimes \eta(a)$. 
    \item In good events, after running regression on  $ \phi(s) \otimes \eta(a)$ and getting $\hat M$, we choose an action following $a_h =\argmax_{a}\hat \eta(a)^{\top}\hat M \hat \phi(a_{0:h-1}) $. 
    \item When we choose the optimal action in bad events, using data $\{\eta(a'),y_{a'}\}_{a'=1}^{|\bar \Acal|}$, we can exactly estimate $y_a$ for any $a\in \Acal$. Thus, the procedure $\max_{a \in \Acal}y_a$ in bad events still works. 
\end{itemize}

==> history.tex <==
\section{M-memory}

Our goal is to learn a policy value of a stationary m-memory policy $\pi: \Hcal \times \Ocal \to \Delta(\Acal)$ where $\Hcal =\prod_{i=0}^{M-1} \Ocal$. The policy value is defined as 
\begin{align*}
    V^{\pi}(s_0) = \sum_{h=0}^{\infty} \gamma^{h} \EE[r_h \mid a_0 \sim \pi_0(h_0),\cdots, a_{M-1} \sim \pi_{M-1}(h_{M-1}), a_M\sim \pi(h_M),\cdots,   ]
\end{align*}
where $h_M=(o_0,\cdots,o_{M-1})$. Here, $\{\pi_k\}_{k=0}^{M-1}$ is a set of history-dependent policies before executing $\pi$, i.e., 
\begin{align*}
    \pi_k : \prod_{t=0}^{k} \Ocal \to \Delta(\Acal).  
\end{align*}
We want to learn $\pi$ and $\{\pi_k\}_{k=0}^{M-1}$ maximizing the policy value over the policy class. 

The algorithm is as follows. 
\begin{itemize}
    \item Fix episode $n$. 
    \item For each $0\leq i\leq M-1$, collect data: 
    \begin{align*}
        (s^{(i)} , a^{(i)}, h^{(i)},o^{(i)}, r^{(i)},o^{'(i)} )  \sim   d^{\bar \pi^{n}}_i(\cdot),\, \bar \pi^{n}= \{U(\Acal),\cdots,U(\Acal)\}. 
    \end{align*}
    This means we execute uniform actions $i+1$ times. Note $h^{(i)}$ is a set of observations up to time step $i$. So $h^{(i)}=(o_{0},\cdots, o_{i-2})$ and we can regard $s^{(i)},o^{(i)},o^{'(i)}$ as $s_i,o_i,o_{i+1}$, respectively, when executing $U(\Acal)$. 
    
  Similarly, we collect data: 
    \begin{align*}
        (\bar s, \bar h) \sim  \sum_{k=M}^{\infty} \gamma_k d^{\bar \pi^{n}}_k(\cdot),  \bar \pi^{n} =\{U(\Acal),\cdots,U(\Acal),\pi,\cdots,\pi,\cdots\},\quad  (\bar a, \bar o, \bar r,\bar o')\sim P(\cdots \mid  \bar s || U(\Acal))
    \end{align*}
Note $ d^{\bar \pi^{n}}_k(s,h)$ is a marginal distribution of 
$(s_1,o_1,s_2,\cdots, )$
with respect to $s_k$ and $(o_{k-M},\cdots,o_{k-1})$ when executing $\bar \pi^n$. 
    
    
    Here, we have a set of functions:
    \begin{align*}
      i \in [0,\cdots, M-1]    f_i : \Ocal \times \{\prod_{k=0}^{i-1} \Ocal\} \to \RR, f:  \Ocal \times \Hcal \to \RR. 
    \end{align*}
    Then, define Bellman error 
    \begin{align*}
      i \in [0,\cdots, M-1];\quad  \sigma^n_i(\pi, \{\pi_i\} ,f,\{f_i\}) = \EE_{\Dcal_n}\left[f_i(o^{(i)} ,h^{(i)})-\frac{I(a^{(i)}= \pi^{n}_i(o^{(i)},h^{(i)}))}{1/|\Acal|}(r^{(i)}+ \gamma f_i(o^{(i+1)} ,h^{(i+1)}))\right]
    \end{align*}
    ($f_M =f$) and
     \begin{align*}
   \sigma^n(\pi, \{\pi_i\} ,f,\{f_i\}) = \EE_{\Dcal_n}\left[f(\bar o ,\bar h)-\frac{I(\bar a= \pi^{n}(\bar o,\bar h))}{1/|\Acal|}(\bar r+ \gamma f(\bar o',\bar h'))\right]
    \end{align*}
\end{itemize}
 We update  a policy as follows: 
\begin{align*}
    (\pi^{n+1}, \{\pi^{n+1}_i\} ):= \argmax_{f,\{f_i\},\pi,\{\pi_i\}  }\EE_{o_0 \sim Z(s_0)}[f(o_0) ]
\end{align*}
such that 
\begin{align*}
      \sum_{p=0}^{n} \sigma^p (\pi, \{\pi_i\} ,f,\{f_i\})^2 \leq \delta,      \quad   \sum_{p=0}^{n} \sigma^p_i(\pi, \{\pi_i\} ,f,\{f_i\})^2 \leq \delta. 
\end{align*}


\subsection{Analysis}

I generally fix an episode $n$ from now on and drop an index. So, $\pi,f$ are actually indexed by $n$.  

\paragraph{Optimism}
We introduce bridge functions. For $\pi^{\diamond}= \{\{\pi_i\}_{i=0}^{M-1},\pi\}$, we define bridge functions: 
\begin{align*}
    &g^{\pi^{\diamond}}:\Ocal \times \Hcal \to [-C,C];  \EE_{o\sim Z(s)}[g^{\pi^{\diamond}}(o,h)]  =V^{\pi^{\diamond}}(s,h),  \\
    &V^{\pi^{\diamond}}(s,h):= \EE[\sum_k \gamma ^k r_k \mid o_0\sim Z(s), a_0 \sim \pi(o_0,h) ,\cdots,\pi,\cdots ] 
\end{align*}
and for each $0\leq i\leq M-1$, 
\begin{align*}
       &g^{\pi^{\diamond}}_i:\Ocal \times \{ \prod_{t=0}^{i-1} \Ocal\} \to [-C,C];   \EE_{o\sim Z(s)}[g^{\pi^{\diamond}}_i(o,h)]  = V^{\pi^{\diamond}}_i(s,h), \\
       &V^{\pi^{\diamond}}_i(s,h)=\EE[[\sum_k \gamma ^k r_k \mid o_0\sim Z(s), a_0  \sim \pi_i(h), \cdots, a_{M-1-i} \sim \pi_{M-1},a_{M-i} \sim \pi,\cdots,\pi ,\cdots ]. 
\end{align*}
Let's say we have realizability of $V^{\pi^{\diamond}}$ and $\{V^{\pi^{\diamond}}_i\}_{i=0}^{M-1}$ for any possible policy. 

\paragraph{After Optimism}
Then, since we have the optimism, the regret is upper-bounded by 
\begin{align*}
    &\EE_{o_0 \sim Z(s_0)}[f_0(o_0)]-V^{\pi^{\diamond}}(s_0)\\
    &= \sum_{k=0}^{M-1} \gamma^k\{\EE_{(s,a,h)\sim d^{\pi^{\diamond}}_k,o \sim z(s), r=r(s,a) }[f_k(o,h)-r(s,a)-\gamma \EE_{s'\sim T(s,a),o'\sim z(s')}[ f_{k+1}(o',h')  ] ] \} + \\
    &+\sum_{k=M}^{\infty} \gamma^k\{\EE_{(s,a,h)\sim d^{\pi^{\diamond}}_k,o \sim z(s), r=r(s,a) }[f(o,h)-r(s,a)-\gamma \EE_{s'\sim T(s,a),o'\sim z(s')}[ f(o',h')  ] ] \}
\end{align*}
(Recall $f,\pi$ are indexed by $n$) 
Here,  we show how to analyze the second term. The firs term is similarly analyzed. 

We can see $d^{\pi^{\diamond}}_k(s,h)$ has a low-rank structure by going back to $M+1$ steps: 
\begin{align*}
     d^{\pi^{\diamond}}_k(s,h)&=\int p(s,h\mid s^- || \pi,\cdots,\pi)d^{\pi^{\diamond}}_{k-M}(s^-)d(s^-)\\
      &=\int p(s,h\mid s^- || \pi,\cdots,\pi)T(s^{-}\mid s^{\dagger},a^{\dagger})d^{\pi^{\diamond}}_{k-M-1}(s^{\dagger},a^{\dagger})d(s^{\dagger},a^{\dagger},s^-) \\ 
         &=\{\int p(s,h\mid s^- || \pi,\cdots,\pi)\mu(s^{-})d(s^-)\}^{\top} \int \phi( s^{\dagger},a^{\dagger})d^{\pi^{\diamond}}_{k-M-1}(s^{\dagger},a^{\dagger})d(s^{\dagger},a^{\dagger}).
\end{align*}
Then, for any $Z(s,h) \in [\Scal\times \Hcal \to \RR]$, we have 
\begin{align*}
      \sum_{k=M}\gamma^k \EE_{d^{\pi^{\diamond},n}_k(s,h)}[Z(s,h)]&= \{\int f(s,h) p(s,h\mid s^- || \pi,\cdots,\pi)\mu(s^{-})d(s^-,s,h)\}^{\top} \int \phi( s^{\dagger},a^{\dagger})d^{\pi^{\diamond}}_{k-M-1}(s^{\dagger},a^{\dagger})d(s^{\dagger},a^{\dagger}) \\ 
       &\leq |\sum_{k=M}\gamma^k \EE_{d^{\pi^{\diamond},n}_{k}(s,h)}[Z(s,h)]| \times \|\sum_{k=M}\gamma^k  \EE_{d^{\pi^{\diamond},n}_{k-M-1}(s,a)}[ \phi( s,a) ] \|_{\Sigma^{-1}_n}
\end{align*}
where $\Sigma_n= \sum_{t=0}^{n-1}\sum_{k=M} \gamma^k \EE_{d^{\pi^{{\diamond},t}}_{k-M-1}(s,a)} \EE[\phi \phi^{\top}(s,a) ]$. (Cumulative sum of the covariance matrix up to episode $n-1$. Here, we use $t$ to denote episode $t$.) In our context, we need to set 
\begin{align*}
    Z(s,h) = \EE_{o \sim Z(s),a \sim \pi(s,h)}[f(o,h) -r(s,a)-\gamma \EE_{s'\sim T(s,a), o'\sim z(s') }[f(o',h')] ]. 
\end{align*}

We first analyze the first term: 
\begin{align*}
     |\frac{1}{n}\sum_{t=1}^{n-1} \sum_{k=M}\gamma^k \EE_{d^{\pi^{{\diamond},t}}_k(s,h)}[Z(s,h)]| 
\end{align*}
This is upper-bounded by 
\begin{align*}
     |A|^{M}\times  |\frac{1}{n}\sum_{t=1}^{n-1} \sum_{k=M}\gamma^k \EE_{d^{\bar \pi^t}_k(s,h)}[Z(s,h)]| 
\end{align*}
Recall 
\begin{align*}
    \bar \pi^t &= \{U(\Acal),\cdots, U(\Acal),\pi^{t},\cdots \}, \quad  \pi^{\diamond,t} = \{\pi^{t}_0,,\cdots,\pi^{t}_{M-1},\pi^{t},\cdots \} \\ 
\end{align*}
Since we have a control over
\begin{align*}
     |\frac{1}{n}\sum_{t=1}^{n-1} \sum_{k=M}\gamma^k \EE_{d^{\bar \pi^t}_k(s,h)}[Z(s,h)]| 
\end{align*}
the first term is upper bounded. 

The second term is uppper bounded by eliptical potential lemma. 


==> main_document/main_check_point.tex <==
\section*{Checklist}




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
     \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We explicitly list up assumptions. }
  \item Did you discuss any potential negative societal impacts of your work?
     \answerNA{Given the theoretical focus of our work, we do not foresee any negative social impacts specific to our work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \answerYes{}
        \item Did you include complete proofs of all theoretical results?
     \answerYes{Due to the page-limit, most of the proof is deferred to Appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
   \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
\answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
\answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?\answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
   \answerNA{}
  \item Did you mention the license of the assets?
   \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
\answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
\answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
\answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}


\end{enumerate}


==> pomdp-deterministic-large.tex <==
\def\usebigfont{1}
\input{neurips_2022}
